Can Your Context-Aware MT System Pass the DiP Benchmark Tests? : Evaluation Benchmarks for Discourse Phenomena in Machine Translation

Despite increasing instances of machine translation (MT) systems including contextual information, the evidence for translation quality improvement is sparse, especially for discourse phenomena. Popular metrics like BLEU are not expressive or sensitive enough to capture quality improvements or drops that are minor in size but significant in perception. We introduce the first of their kind MT benchmark datasets that aim to track and hail improvements across four main discourse phenomena: anaphora, lexical consistency, coherence and readability, and discourse connective translation. We also introduce evaluation methods for these tasks, and evaluate several baseline MT systems on the curated datasets. Surprisingly, we find that existing context-aware models do not improve discourse-related translations consistently across languages and phenomena.

==> error-examples.tex <==
\begin{table}[t]
%    \small
    \centering
    \scalebox{0.85}
  { \begin{tabular}
    {l|c|c|c|c}
 Error type & Source text & Translation & Error & Correction\\
 
 Gender Copy & \textit{Mir wurde \textbf{diese Wohnung} in Earls Court gezeigt, und \textbf{sie} hatte ...} & \textit{she} & \textit{it} \\
 Named Entity & - & \textit{... \textbf{Lady Liberty} is stepping forward. \textbf{It} is meant to be carrying the torch of liberty ...} & \textit{It} & \textit{she} \\
 
    \end{tabular}}

    \caption{}
    
    \label{tab:error-examples}
\end{table}


==> evaluation.tex <==
\begin{table*}
\centering
\small
\tabcolsep=0.1cm
\setlength\extrarowheight{-10pt}
\begin{tabular}{l|c|cccc|ccccccc|c|cccccc}  
%\toprule
& & \multicolumn{4}{c|}{\textbf{Anaphora}} & \multicolumn{7}{c|}{\textbf{Lexical Consistency}} & \textbf{C\&R} & \multicolumn{6}{c}{\textbf{Discourse Connectives}}\\ [+0.3em]
\textbf{Models} & \textbf{BLEU} & \textbf{Rk} & GC & NE & Lg & \textbf{Rk} & Acc & Syn & Rel & Om. & NE & Rand & \textbf{Rk}  & \textbf{Rk} & Acc. & ANY & Om. & Syn & Mis \\
%& & & & \% & \% & \% &  &\% &\% &\% &\% &\% &\% &  & & \%& \%& \%&  \%& \%  \\
\midrule
\multicolumn{18}{c}{\textbf{De-En}}
\\[+0.3em]

{\sts} & 31.65 & \textbf{1} & 63 & 25 & 12 & \textbf{3}  & 36.85 & 38 & 19 & 29 & 5 & 9 & \textbf{1} & \textbf{2} & 50.46 & 78.90 & 76 & 24 & 0\\
{\concat} & \textbf{31.96} & \textbf{2}  & 55 & 33 & 11 & \textbf{1}  & 42.30 & 38 & 15 & 23 & 4 & 19 &\textbf{3} & \textbf{4} & 46.79 & 75.23 & 68 & 32 & 0\\
{\anap} & 29.94 & \textbf{5} & 42 & 17 & 41 & \textbf{2} & 38.14 & 46 & 21 & 21 & 4 & 8 & \textbf{4} & \textbf{3} & 50.46 & 76.5 & 75 & 25 & 0\\
{\han} & 29.22 & \textbf{3} & 44 & 22 & 33 & \textbf{4} & 36.21  & 35 & 22 & 30 & 4 & 7 & \textbf{5} &\textbf{5} & 46.79 & 67.89 & 72  & 28 & 0\\
{\san} & 29.32  & \textbf{4} & 27 & 27 & 46 & \textbf{5} & 35.57 & 38 & 19 & 24 & 5 & 14 & \textbf{2} & \textbf{1} & 52.29 & 76.15 & 67 & 33 & 0\\

\midrule
\multicolumn{18}{c}{\textbf{Fr-En}}
\\[+0.3em]

{\sts} & 35.12 & \textbf{1} & 0 & 67 & 33 & \textbf{2} & 36.04 & 43 & 19 & 19 & 0 & 19 & \textbf{2} &\textbf{2} & 48.62 & 75.23 & 53 & 44 & 2 \\
{\concat}  & \textbf{35.34} & \textbf{3} & 42 & 14 & 44 & \textbf{5} & 30.81 & 35 & 25 & 15 & 0 & 25 & \textbf{3} & \textbf{1} & 48.62 & 76.15 & 47 & 50 & 3 \\
{\anap} & 34.32 & \textbf{2} & 50 & 50 & 0 & \textbf{3} & 35.46 & 55 & 10 & 5 & 5 & 25 & \textbf{4} & \textbf{5} & 46.79 & 68.81 & 53 & 41 & 6 \\
{\han} & 33.30 & \textbf{5} & 50 & 0 & 50 & \textbf{1} & 36.21 & 48 & 26 & 4 & 0 & 22  & \textbf{5} & \textbf{3} & 46.79 & 71.56 & 53 & 43 & 3 \\
{\san} & 33.48 & \textbf{4} & 43 & 29 & 28 & \textbf{4}  & 30.81 & 44 & 12 & 12 & 0 & 32 & \textbf{1} & \textbf{4} & 46.79 & 70.64 & 56 & 41 & 2 \\

\midrule
\multicolumn{18}{c}{\textbf{Ru-En}}
\\[+0.3em]

{\sts} & 23.88 & \textbf{2}  & 37 & 37 & 26 & \textbf{2} & 10.33 & 21 & 9 & 27 & 21 & 21 & \textbf{1} & \textbf{1} & 40.17 & 76.92 & 59 & 28 & 12 \\
{\concat} & 24.56 & \textbf{4} & 29 & 46 & 25 & \textbf{2} & 10.33 & 15 & 8 & 15 & 18 & 44 & \textbf{3} & \textbf{4} & 35.04 & 75.08 & 61 & 32 & 6 \\
{\anap} & \textbf{27.66} & \textbf{1} & 29 & 46 & 25 & \textbf{1} & 13.68 & 15 & 0 & 26 & 15 & 44 & \textbf{2} & \textbf{2} & 39.32 & 68.38 &   63 & 30 & 7 \\
{\han} & 25.11 & \textbf{3} & 31 & 48 & 21 & \textbf{4} & 5.58 & 11 & 8 & 19 & 19 & 41 & \textbf{5} & \textbf{5} & 33.34 & 57.26 & 76 & 21 & 3 \\
{\san} & 26.24 & \textbf{5} & 32 & 44 & 24 & \textbf{3}  & 8.37 & 6 & 9 & 24 & 18 & 42 & \textbf{4} & \textbf{3} & 39.32 & 64.96 & 62 & 28 & 9 \\

\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{{BLEU scores and evaluation results on the DiP benchmark testsets. \textbf{R}an\textbf{k}ings of the models are in bold. Each set of rankings is followed by the results of the manual analysis on a subset of the translation data. The percentages for the following types of errors are reported: Anaphora - instances of \textbf{G}ender \textbf{C}opy, \textbf{N}amed \textbf{E}ntity and \textbf{L}an\textbf{g}uage specific errors; Lexical Consistency - \textbf{Acc}uracy, \textbf{Syn}onyms, \textbf{Rel}ated words, \textbf{Om}issions, \textbf{N}amed \textbf{E}ntity, \textbf{Rand}om translation; Discourse Connectives - \textbf{Acc}uracy, percentage of samples with \textbf{ANY} candidate connective, \textbf{Om}issions, \textbf{Syn}onyms, \textbf{Mis}translations.  For \textbf{C}oherence \&  \textbf{R}eadability, only rankings are shown.  }}

\label{tab:eval-results}
\end{table*}

\begin{comment}

The BLEU scores, model rankings and results\footnote{See Appendix for raw scores used to produce rankings and examples for each error category.} on each of the DiP testsets given in Table \ref{table:testsets} for De-En, Fr-En and Ru-En translation tasks are given in Table \ref{tab:eval-results}. 
% In the following subsections, we provide the manual analysis for a subset of the translations for each of the discourse phenomena. See {Appendix} for the raw scores that produced the rankings.
% \subsection{BLEU scores}
%As displayed in the table, 
We observe a variability in BLEU scores across models.
{In contrast to increases in BLEU for selected language-pairs and datasets reported in the  published work, incorporating context within elaborate context-dependent models decreases BLEU scores for Fr-En and De-En.} \concat, the simple concatenation-based model,  achieves the best result out of all of the tested models. This shows that context knowledge is indeed helpful for improving the BLEU. 



%However, the three elaborate architectures seem to fail in representing this knowledge appropriately. 

%\shafiq{Note that \citet{bawden-etal-2018-evaluating} also evaluate a \concat\ model in the En-Fr task and report inferior results  compared to their dedicated (source) context encoder model. We suspect this is due to the architectural differences as they use a recurrent-based seq2seq model, whereas Transformers are arguably more flexible in capturing contextual dependecies \cite{NIPS2017_7181_vaswani}}. \alert{we may exclude this if we need space} 

For Ru-En, dedicated context-aware models improve the performance. In particular, \anap\ achieves the highest score of all - interestingly, it has been trained and tested on En-Ru in the original paper \cite{voita-etal-2018-context}. This shows that complex architectures might only be useful for certain types of languages (such as highly inflected languages, like Russian). 

\end{comment}

% Another possible cause is that the context-aware models might be helpful in discovering vital relations in the comparatively small size of the dataset, which are learned per se even by a simple model on a larger dataset. 

%On a general note, our results show that dedicated models do not live up to the promise of better representing context phenomena.
%as judged by overall translation quality. 
{In general, our findings match the conclusions from \citet{context-study} regarding the lack of satisfactory performance gains in context-aware models. However, our results stress that the problem is not caused by context being unhelpful or unrepresented by BLEU, but rather by the faulty behavior of the models themselves, as the simple contextual model \concat\ is able to beat both context-aware models as well as a sentence-level model.}
% \blue{Our findings match the conclusions from \citet{context-study}.}




% \subsection{Anaphora}

% \begin{table}[]
% \centering
% \small
% \begin{tabular}{c|c|c}
% French & German & Russian  \\
% \midrule
%   \citet{miculicich-etal-2018-document} &  Sentence2Sentence &  \\
%   Sentence2Sentence  & \citet{miculicich-etal-2018-document}&  \\
%     \citet{voita-etal-2018-context} & S-Concat &  \\
%   \citet{zhang-etal-2018-improving}*  & \citet{zhang-etal-2018-improving} & \\
%   S-Concat*  & \citet{voita-etal-2018-context} & \\
        
        
%     \end{tabular}
%     \caption{Rankings (best to worst) of the models in terms of pronoun translation accuracies *\textit{ex-aequo}}
%     \label{results:anaphora}

% \end{table}
\vspace{-0.3em}
\subsection{Anaphora}

%{The ranking of the models based on their performance on the anaphora testet is given in Table \ref{tab:eval-results}. 

%We also manually analyze a subset of the anaphora benchmark translations to discover the linguistic phenomena which occur, especially in the incorrectly translated examples. Table \ref{table:datasets_anaphora-analysis} contains the aggregated results.
%We have identified the following tendencies.
We observed the following types of errors:

\begin{description}[leftmargin=0pt,itemsep=-0.3em]
\vspace{-0.7em}
\item [\Ni Gender Copy.]  
%This is a tendency to carry over gender from gender marked pronouns inherent in Fr/De/Ru languages. 
Translating from Fr/De/Ru to En often requires the `flattening' of gendered pronouns to \textit{it}, since Fr/De/Ru assign gender to all nouns. In many cases the machine translated pronouns tend to {(mistakenly)} agree with the source language. For example, % the sentence\textit{Mir wurde \textbf{diese Wohnung} in Earls Court gezeigt, und \textbf{sie} hatte ...}
{\textit{\textbf{diese Wohnung} in Earls Court..., und \blue{\textbf{sie}} hatte...} is translated to : \textit{\textbf{apartment} in Earls Court, and \red{\textbf{she}} had...},} a version which upholds the female gender expressed in \textit{sie}, instead of translating it to \textit{it}. 
%Ideally, the English text should have the pronoun \textit{it} instead of \textit{she}. 
{This was the most common error, except for Ru-En, where Named Entity errors were slightly more prevalent.}

% \textbf{Neuter.} This is a tendency to replace male and female personal pronouns with a neutral 'it' or plural 'they'. 

\item[\Nii Named Entity.] A particularly hard problem is to infer gender from a named entity, \eg\ %\textit{... \textbf{Lady Liberty} is stepping forward. \textbf{She} is meant to be carrying the torch of liberty ...} 
{\textit{\textbf{Lady Liberty}...\blue{\textbf{She}} is meant to...}}- \textbf{she} is wrongly translated to \red{\textbf{it}}. Such  examples demand higher inference abilities such as world knowledge {(\eg\ distinguish male/female names).}
%(i.e., which names are male/female names? Which nouns are necessarily male/female?).

\item[\Niii Language specific phenomena.] {Pronouns can be ambiguous in the source language.}
%These are the phenomena specific to a language, where ambiguous pronouns can create additional problems for the model. 
For example in German, the pronoun 
% \textit{ihr} can mean \textit{her}, \textit{their}, or \textit{your}, while
\textit{sie} can mean both \textit{she} and \textit{you}, depending on capitalization, sentence structure, and context. This type of error often appears in the context-aware models, while being relatively rare for the {\sts\ model}. %vanilla Transformer.


\vspace{-0.7em}
\end{description}


In summary, we observe that surprisingly, \sts\ is translating pronouns comparatively well - outperforming all other De-En and Fr-En models, and only giving way to \anap\ in Ru-En. However, for De-En, \anap\ proved to be the worst contender so there is no clear tendency for this system's performance. \san\ is consistently poor in this task. The success of the {\sts\ model}
%\vanilla Transformer
can be explained by its tendency to use \textit{it} as the default pronoun, which statistically appears most often due to the lack of grammatical gender in English. More variability in pronouns occurs in the outputs of the context-aware models, but this does not contribute to a greater success.







\vspace{-0.3em}
\subsection{Lexical Consistency}




 
Our manual inspection of the lexical chains shows the following tendencies:


\begin{description}[leftmargin=0pt,itemsep=-0.3em]
\vspace{-0.5em}
\item [\Ni Synonym \& related word.] Words are exchanged for their synonyms (\textit{poll} - \textit{survey}), hypernyms/hyponyms  (\textit{ambulance} - \textit{car}) or related concepts (\textit{wine} - \textit{vineyard}).

%For lexical consistency, synonymous translations are not welcome since we expect all words in a lexical chain to be translated exactly the same.

\item [\Nii Named Entity.] Models tend to distort proper names and translate them inconsistently. For example, the original name  \textit{Füchtorf} (name of a town) gets translated to \textit{feeding-community}.

\item [\Niii Omission.] Occurs when words are omitted altogether from the lexical chain.

\vspace{-0.7em}
\end{description}

{The overall low quality of Russian translations contributes to the prevalence of \textbf{Rand}om translations, and the necessity to transliterate named entities increases NE errors, compared to other languages.}
We do not observe a decisive winner across models, but \concat\ and  \sts\ are again successful {on average, taking the first or second place in all tested languages.}
%taking the first and second place in De-En and Fr-En, respectively.


\vspace{-0.3em}
\subsection{Discourse Connectives}


In benchmark outputs, we observed mostly \textbf{omissions} of connectives (disappears in the translation), \textbf{synonymous translations} (\eg\  \textit{Naldo is \blue{\textbf{also}} a great athlete on the bench} - \textit{Naldo's ``great sport" on the bank, \red{\textbf{too}}.}), and \textbf{mistranslations}.

The ranking shows that \sts\ models are on average the most accurate and {omit the connectives less often}. \han\ models had a clear tendency to omit connectives and were found to be consistently poor in this task. Other models show no clear tendency. 

\vspace{-0.3em}
\subsection{Coherence and Readability}
We identified the following types of coherence and readability errors (Appendix has more examples).

%\basia{Manual qualitative analysis allows us to identify core reasons for loss of coherence. In Appendix we present examples of the errors.}

%\begin{description}[leftmargin=0pt,itemsep=-0.3em]
%\vspace{-0.5em}
\noindent \textbf {\Ni Inconsistency}. As in
\citet{somasundaran-etal-2014-lexical}, we observe that inconsistent translation of words across sentences (in particular named entities) breaks the continuity of meaning.

\noindent \textbf {\Nii Translation error.} Errors at various levels  spanning from ungrammatical fragments to model hallucinations introduce fragments which bear little relation to the whole text \cite{smith-etal-2016-trouble}. {An example of this:}
\blue{Reference}: \textit{There is huge applause for the Festival Orchestra, who appear on stage for the first time – in casual leisurewear in view of the high heat.} \red{Translation}: \textit{There is great applause for the solicitude orchestra , which is on the stage for the first time, with the heat once again in the wake of an empty leisure clothing.}

%\vspace{-0.7em}
%\end{description}


% \red{Translation}: \textit{Farmers are allowed to start annual cage care on Monday.}
% \blue{Reference}: \textit{On Monday farmers are allowed to start the annual hedge bank maintainance.}



From the ranking in Table \ref{tab:eval-results} (C\&R), we see that \sts\ is the most coherent model for De-En and Ru-En. For Fr-En however, we observe an advantage of the context-aware model - \san, which received high {ranking} in De-En too.
The example of \san\ shows that a model can deal relatively well with one aspect of discourse translation (coherence) and do badly in another (anaphora). 

%Analysis shows that the leading cause for loss of coherence is \emph{disconnected sentences}, for example, %\blue{Reference:} %\textit{``Before his appointment, Geoffrey Ross Pyatt was an ambassador in Kiyv. During his mission, the Maydan events and state coup happened, reminds Gazeta.Ru.''} 
%\red{Translation:} \textit{``Before appointing Greece, Jeffrey Pyett was the US ambassador to Kiev. When it came to the Maidan and the coup in 2014 , it was a newspaper.''}


%\red{Translation}: ``\textit{We are shining information}''. \blue{Reference}: ``\textit{We warmly welcome this announcement}''. 
%\red{Translation:} \textit{``Before appointing Greece, Jeffrey Pyett was the US ambassador to Kiev. When it came to the Maidan and the coup in 2014 , it was a newspaper.''} \blue{Reference:} \textit{``Before his appointment, Geoffrey Ross Pyatt was an ambassador in Kiyv. During his mission, the Maydan events and state coup happened, reminds Gazeta.Ru.''}}
%Other errors include \emph{nonsensical translation} of a phrase in a context, and \emph{ungrammatical} translations\footnote{See Appendix for more examples.}.}    



